How reliable are automated X-ray reflection spins of supermassive black holes? A methodological study of 41 AGN with simultaneous \xmm\ and \nustar\ data

This is a methodological study: we test how reliable black hole spins from an automated, uniform reflection analysis are, not how spins are distributed. We fit one simultaneous XMM-Newton EPIC-pn and NuSTAR observation of each of 41 AGN with relxillCp, a distant reflector and a warm-Comptonisation soft excess, using quality criteria fixed in advance, 20 starting points, spin profiles scanned in both directions and two-dimensional (spin, inclination) grids. We test whether the relativistic reflection is detected, and test every result against four changes to the model, two sensitivity tests, two alternative models (a high-density disc and a lamppost corona) and simulations. The disc reflection is not detected in 21 of the 41 sources, and 5 sources pass all checks. Their 90% spin regions are 1 lower bound (NGC 4051, a*>0.75), 1 upper bound, 2 regions in separate pieces and 1 unconstrained profile; none is a two-sided interval. The accepted fits lie at 32-56 deg. No constrained region keeps its type under all of the inclination limit, the removal of pn data below 3 keV, and the two alternative models, so the spin depends on how the soft excess and the corona are modelled. In two accepted sources, including NGC 4051, the disc component is detected mainly below 2 keV rather than in the iron band. Of the 18 sources accepted by a previous version of this analysis without a soft-excess component, 14 are not accepted, 11 because their disc reflection is not detected; none of the accepted fits is now edge-on (10 of 18 before). In simulations with known spin the 90% regions contain the true spin in 0.82 of cases when the model is correct; fitting the previous model to spectra simulated from the new one gives spuriously high spins and, for one of two templates, edge-on inclinations. The sample is not complete, and we make no statement about the spin distribution.

==> tab_v9_arms_a.tex <==
ESO~141$-$G055 & $<$0.76 (43) & $<$0.76 & all & $<$0.78 & $<$0.77 \\
NGC~1566 & [0.29, 0.83] $\cup$ $>$0.86 (39) & [0.12, 0.51] $\cup$ [0.74, 0.76] & $>$0.35 & $>$0.48$^{\ast}$ & [0.13, 0.81] $\cup$ $>$0.92 \\
NGC~4051 & $>$0.75 (32) & [0.03, 0.36] $\cup$ $>$0.88 & $>$0.77 & $>$0.70 & $>$0.75 \\
NGC~7469 & all (56) & all & all & all & all \\
Swift~J2127.4+5654 & [0.37, 0.72] $\cup$ $>$0.88 (39) & $>$0.94 & $>$0.40 & [0.77, 0.81] $\cup$ $>$0.82 & $>$$-$0.08 \\
\midrule
ESO~362$-$G18 & all$^{\ast}$ (3) & [0.55, 0.94] $\cup$ $>$0.98$^{\ast}$ & $>$0.81$^{\ast}$ & $>$0.78$^{\ast}$ & $>$0.81$^{\ast}$ \\
PDS~456 & $<$$-$0.29$^{\ast}$ (87) & all$^{\ast}$ & all$^{\ast}$ & all$^{\ast}$ & all$^{\ast}$ \\
Fairall~9 & [$-$0.84, 0.83] $\cup$ $>$0.87 (33) & [$-$0.41, 0.91] & all & $<$0.14 $\cup$ [0.45, 0.78] $\cup$ $>$0.82 & [$-$0.83, 0.83] $\cup$ $>$0.86 \\
Ton~S180 & $>$0.53$^{\ast}$ (80) & $>$$-$0.28$^{\ast}$ & $>$0.53$^{\ast}$ & $>$0.62 & $>$0.54$^{\ast}$ \\
Ark~120 & [0.02, 0.70]$^{\ast}$ (87) & [0.17, 0.68]$^{\ast}$ & $>$0.10$^{\ast}$ & [0.09, 0.79] & [0.04, 0.70]$^{\ast}$ \\


==> tab_v9_arms_b.tex <==
ESO~141$-$G055 & $<$$-$0.16 & $>$0.50 & $>$0.94 (80) & all (62) \\
NGC~1566 & [0.23, 0.85] $\cup$ $>$0.85 & all$^{\ast}$ & [0.90, 0.97]$^{\dagger}$$^{\ast}$ (87) & [0.01, 0.53]$^{\ast}$ (31) \\
NGC~4051 & $>$0.75 & all & $>$0.82$^{\ast}$ (3) & [0.89, 0.91] $\cup$ $>$0.92 (34) \\
NGC~7469 & all & all & $<$0.93$^{\dagger}$$^{\ast}$ (87) & $<$0.17 (57) \\
Swift~J2127.4+5654 & $>$$-$0.58 & $<$0.72 & $<$0.67$^{\ast}$ (3) & $>$$-$0.43 (39) \\
\midrule
ESO~362$-$G18 & all$^{\dagger}$$^{\ast}$ & all$^{\ast}$ & $>$0.93$^{\ast}$ (3) & --$^{\ast}$ (5) \\
PDS~456 & all & all & $<$0.06 (33) & all (77) \\
Fairall~9 & [$-$0.84, 0.83] $\cup$ $>$0.86 & $<$0.56 & [0.92, 0.97]$^{\ast}$ (87) & all (29) \\
Ton~S180 & $<$0.95 & $>$$-$0.14 & $>$0.78 (83) & $>$0.38 (78) \\
Ark~120 & $<$0.71 $\cup$ $>$0.95 & $<$0.69 & $>$0.93$^{\dagger}$$^{\ast}$ (87) & $<$0.11 (39) \\


==> tab_v9_census.tex <==
ESO~141$-$G055 & Y & 1484/1444 & 2.3e-01 & p$\geq$0.01 & 41.0 & -- & 43 & $<$0.76 & Y \\
NGC~1566 & Y & 1475/1514 & 7.6e-01 & p$\geq$0.01 & 73.5 & -- & 39 & [0.29, 0.83] $\cup$ $>$0.86 & Y \\
NGC~4051 & Y & 649/613 & 1.5e-01 & p$\geq$0.01 & 98.7 & -- & 32 & $>$0.75 & Y \\
NGC~7469 & Y & 917/841 & 3.4e-02 & p$\geq$0.01 & 73.2 & -- & 56 & all & Y \\
Swift~J2127.4+5654 & Y & 923/893 & 2.4e-01 & p$\geq$0.01 & 92.8 & -- & 39 & [0.37, 0.72] $\cup$ $>$0.88 & Y \\
1H~0323+342 & Y & 385/430 & 9.4e-01 & p$\geq$0.01 & 12.2 & S & 32 & all & N \\
1H~0419$-$577 & Y & 910/849 & 7.1e-02 & p$\geq$0.01 & 14.4 & P & 3 & $>$$-$0.60 & N \\
3C~382 & Y & 922/905 & 3.4e-01 & p$\geq$0.01 & 7.4 & S & 57 & all & N \\
Ark~120 & Y & 1194/1112 & 4.3e-02 & p$\geq$0.01 & 70.0 & P & 87 & [0.02, 0.70] & N \\
ESO~362$-$G18 & Y & 1211/1153 & 1.1e-01 & p$\geq$0.01 & 0.0 & P,S & 3 & all & N \\
ESO~511$-$G030 & Y & 434/437 & 5.3e-01 & p$\geq$0.01 & 0.0 & S & 9 & all & N \\
Mrk~1040 & Y & 1245/1215 & 2.7e-01 & p$\geq$0.01 & 0.0 & S & 38 & all & N \\
Mrk~110 & Y & 1216/1247 & 7.3e-01 & p$\geq$0.01 & 0.0 & P,S & 87 & all & N \\
Mrk~1501 & Y & 1196/1156 & 2.0e-01 & p$\geq$0.01 & 0.0 & P,S & 3 & all & N \\
Mrk~359 & Y & 677/650 & 2.2e-01 & p$\geq$0.01 & 5.8 & S & 79 & all & N \\
Mrk~509 & Y & 950/925 & 2.8e-01 & p$\geq$0.01 & 7.6 & S & 37 & all & N \\
Mrk~590 & Y & 530/483 & 7.0e-02 & p$\geq$0.01 & 0.0 & P,S & 87 & all & N \\
Mrk~915 & Y & 571/586 & 6.6e-01 & p$\geq$0.01 & 0.1 & S & 11 & all & N \\
NGC~4593 & Y & 662/700 & 8.4e-01 & p$\geq$0.01 & 0.0 & P,S & 3 & all & N \\
NGC~5548 & Y & 1322/1273 & 1.6e-01 & p$\geq$0.01 & 69.0 & P & 3 & $>$0.70 & N \\
PDS~456 & Y & 883/841 & 1.5e-01 & p$\geq$0.01 & 105.6 & P & 87 & $<$$-$0.29 & N \\
RBS~1124 & Y & 955/939 & 3.5e-01 & p$\geq$0.01 & 0.0 & P,S & 87 & all & N \\
RXS~J1131$-$1231 & Y & 658/656 & 4.7e-01 & p$\geq$0.01 & 7.5 & P,S & 87 & all & N \\
HE~1136$-$2304 & Y & 712/612 & 3.1e-03 & expl. & 71.0 & -- & 79 & $<$$-$0.14 & N \\
IC~4329A & Y & 1462/1260 & 6.4e-05 & expl. & 0.0 & P,S & 3 & all & N \\
IRAS~09149$-$6206 & Y & 1367/1201 & 5.8e-04 & expl. & 284.8 & P & 3 & $>$0.79 & N \\
Mrk~766 & Y & 1126/973 & 4.4e-04 & expl. & 161.7 & -- & 71 & $<$0.43 & N \\
Mrk~841 & Y & 1526/1373 & 2.3e-03 & expl. & 8.3 & S & 86 & $>$$-$0.74 & N \\
NGC~3227 & Y & 1462/1235 & 7.6e-06 & expl. & 0.0 & P,S & 3 & all & N \\
NGC~3516 & Y & 1566/1399 & 1.1e-03 & expl. & 124.6 & -- & 4 & [0.06, 0.54] $\cup$ $>$0.997 & N \\
NGC~3783 & Y & 1334/1161 & 2.9e-04 & expl. & 415.4 & P & 3 & [0.68, 0.87] $\cup$ $>$0.90 & N \\
NGC~985 & Y & 508/426 & 3.8e-03 & expl. & 6.6 & P,S & 3 & [0.02, 0.18] $\cup$ $>$0.21 & N \\
3C~120 & Y & 1655/1286 & 1.1e-11 & inad. & 0.0 & P,S & 3 & all & N \\
IRAS~13197$-$1627 & Y & 2278/826 & 5.2e-136 & inad. & 113.7 & P,S & 3 & $<$$-$0.74 & N \\
MCG$-$5$-$23$-$16 & Y & 2140/1777 & 5.0e-09 & inad. & 25.0 & P & 3 & $>$0.72 & N \\
MCG$-$6$-$30$-$15 & Y & 1186/948 & 1.9e-07 & inad. & 0.0 & P,S & 87 & all & N \\
Mrk~335 & Y & 803/484 & 3.3e-18 & inad. & 72.3 & S & 50 & $<$$-$0.33 & N \\
NGC~1365 & Y & 3220/1294 & 8.3e-165 & inad. & 523.2 & P & 3 & $>$0.97 & N \\
NGC~2992 & Y & 4748/1620 & 6.7e-304 & inad. & 0.0 & P,S & 3 & all & N \\
NGC~4151 & Y & 4421/2124 & 2.2e-163 & inad. & 2721.4 & -- & 27 & $>$0.99 & N \\
NGC~7314 & Y & 1992/1428 & 2.2e-21 & inad. & 352.8 & N,P,S & 3 & [0.76, 0.90] & N \\
Fairall~9 & N & 1211/1224 & 6.0e-01 & p$\geq$0.01 & 24.7 & -- & 33 & [$-$0.84, 0.83] $\cup$ $>$0.87 & N \\
Ton~S180 & N & 693/726 & 8.0e-01 & p$\geq$0.01 & 16.5 & S & 80 & $>$0.53 & N \\


==> tab_v9_literature.tex <==
Mrk~359 & $\sim$1.1 & $0.66^{+0.30}_{-0.54}$ & $0.66^{+0.30}_{-0.54}$ & all & disc refl.\ not detected \\
Ark~564 & $\sim$1.1 & $>0.9$ & $>0.9$ & -- & no eligible pair \\
Mrk~766 & 1.8 & $>0.92$ & $>0.92$ & $<$0.43 & exploratory fit \\
NGC~4051 & 1.91 & $>0.99$ & not listed & $>$0.75 & accepted \\
NGC~1365 & $\sim$2 & $>0.97$ & $>0.97$ & $>$0.97 & inadequate fit \\
1H~0707$-$495 & $\sim$2.3 & $>0.94$ & $>0.97$ & -- & no eligible pair \\
MCG$-$6$-$30$-$15 & 2.9 & $0.91^{+0.06}_{-0.07}$ & $>0.65$$^{a}$ & all & inadequate fit \\
NGC~5506 & $\sim$5 & $0.93^{+0.04}_{-0.04}$ & $0.93^{+0.04}_{-0.04}$ & -- & no eligible pair \\
IRAS~13224$-$3809 & $\sim$6.3 & $>0.975$ & $>0.975$ & -- & no eligible pair \\
Ton~S180 & $\sim$8.1 & $>0.98$ & $>0.98$ & $>$0.53 & no eligible pair; comparison fit \\
ESO~362$-$G18 & 12.5 & $>0.92$ & $>0.92$ & all & disc refl.\ not detected \\
Swift~J2127.4+5654 & $\sim$15 & $0.72^{+0.14}_{-0.20}$ & $0.72^{+0.14}_{-0.20}$ & [0.37, 0.72] $\cup$ $>$0.88 & accepted \\
Mrk~335 & 17.8 & $>0.99$ & $>0.91$ & $<$$-$0.33 & inadequate fit \\
Mrk~110 & 25.1 & $>0.99$ & $>0.89$ & all & disc refl.\ not detected \\
NGC~3783 & 29.8 & $>0.88$ & $>0.88$ & [0.68, 0.87] $\cup$ $>$0.90 & exploratory fit \\
1H~0323+342 & 34 & $>0.9$ & $>0.9$ & all & disc refl.\ not detected \\
NGC~4151 & 45.7 & $>0.9$ & $>0.9$ & $>$0.99 & inadequate fit \\
Mrk~79 & 52.4 & $>0.5$ & $>0.5$ & -- & no eligible pair \\
PG~1229+204 & 57 & $0.93^{+0.06}_{-0.02}$ & $0.93^{+0.06}_{-0.02}$ & -- & no eligible pair \\
IRAS~13197$-$1627 & $\sim$64 & $>0.7$ & $>0.7$ & $<$$-$0.74 & inadequate fit \\
3C~120 & 69 & $>0.95$ & $>0.95$ & all & inadequate fit \\
Mrk~841 & $\sim$79 & $>0.52$ & $>0.52$ & $>$$-$0.74 & exploratory fit \\
IRAS~09149$-$6206 & $\sim$100 & $0.94^{+0.02}_{-0.07}$ & $0.94^{+0.02}_{-0.07}$ & $>$0.79 & exploratory fit \\
Ark~120 & 150 & $>0.85$ & $0.64^{+0.32}_{-0.06}$ & [0.02, 0.70] & flagged (P) \\
RBS~1124 & $\sim$180 & $>0.8$ & $>0.236$ & all & disc refl.\ not detected \\
RXS~J1131$-$1231 & $\sim$200 & $0.87^{+0.08}_{-0.15}$ & $0.87^{+0.08}_{-0.15}$ & all & disc refl.\ not detected \\
Fairall~9 & 255 & $0.52^{+0.19}_{-0.15}$ & $0.71^{+0.08}_{-0.09}$ & [$-$0.84, 0.83] $\cup$ $>$0.87 & no eligible pair; comparison fit \\
1H~0419$-$577 & $\sim$340 & $>0.98$ & $>0.98$ & $>$$-$0.60 & flagged (P) \\
H~1821+643 & 4500 & $>0.4$ & $0.62^{+0.22}_{-0.37}$ & -- & no eligible pair \\
IRAS~00521$-$7054 & -- & $>0.77$ & $>0.77$ & -- & no eligible pair \\
Mrk~1501 & -- & $>0.97$ & $>0.97$ & all & disc refl.\ not detected \\


==> tab_v9_othermethods.tex <==
H~1821+643 & continuum & $0.5^{+0.5}_{-0.4}$ & \citet{Capellupo2017} & -- & -- & no eligible pair \\
NGC~3783 & continuum & $0.2^{+0.7}_{-0.9}$ (no disc wind) & \citet{Capellupo2017} & [0.68, 0.87] $\cup$ $>$0.90 & 3 & exploratory fit \\
NGC~3783 & continuum & $0.5^{+0.5}_{-0.4}$ (with disc wind) & \citet{Capellupo2017} & [0.68, 0.87] $\cup$ $>$0.90 & 3 & exploratory fit \\
RXS~J1131$-$1231 & microlensing & $\gtrsim0.8$ & \citet{Chartas2017} & all & 87 & disc refl.\ not detected \\
3C~120 & outflow & $1.00\pm0.15$ & \citet{Daly2019} & all & 3 & inadequate fit \\
Ark~564 & outflow & $1.00\pm0.15$ & \citet{Daly2019} & -- & -- & no eligible pair \\
IC~4329A & outflow & 1.00 & \citet{Daly2019} & all & 3 & exploratory fit \\
Mrk~335 & outflow & $0.81\pm0.15$ & \citet{Daly2019} & $<$$-$0.33 & 50 & inadequate fit \\
Mrk~509 & outflow & 0.44 & \citet{Daly2019} & all & 37 & disc refl.\ not detected \\
Mrk~590 & outflow & 0.88 & \citet{Daly2019} & all & 87 & disc refl.\ not detected \\
Mrk~766 & outflow & 1.00 & \citet{Daly2019} & $<$0.43 & 71 & exploratory fit \\
NGC~1365 & outflow & $1.00\pm0.15$ & \citet{Daly2019} & $>$0.97 & 3 & inadequate fit \\
NGC~2110 & outflow & 0.84 & \citet{Daly2019} & -- & -- & no eligible pair \\
NGC~2992 & outflow & 0.98 & \citet{Daly2019} & all & 3 & inadequate fit \\
NGC~3227 & outflow & 0.83 & \citet{Daly2019} & all & 3 & exploratory fit \\
NGC~3516 & outflow & 0.64 & \citet{Daly2019} & [0.06, 0.54] $\cup$ $>$0.997 & 4 & exploratory fit \\
NGC~4051 & outflow & $1.00\pm0.15$ & \citet{Daly2019} & $>$0.75 & 32 & accepted \\
NGC~4151 & outflow & $0.84\pm0.15$ & \citet{Daly2019} & $>$0.99 & 27 & inadequate fit \\
NGC~5548 & outflow & 0.58 & \citet{Daly2019} & $>$0.70 & 3 & flagged (P) \\
NGC~7469 & outflow & 0.94 & \citet{Daly2019} & all & 56 & accepted \\
PG~1229+204 & outflow & 0.43 & \citet{Daly2019} & -- & -- & no eligible pair \\

